On Relating 'Why?' and 'Why Not?' Explanations

Explanations of Machine Learning (ML) models often address a 'Why?' question. Such explanations can be related with selecting feature-value pairs which are sufficient for the prediction. Recent work has investigated explanations that address a 'Why Not?' question, i.e. finding a change of feature values that guarantee a change of prediction. Given their goals, these two forms of explaining predictions of ML models appear to be mostly unrelated. However, this paper demonstrates otherwise, and establishes a rigorous formal relationship between 'Why?' and 'Why Not?' explanations. Concretely, the paper proves that, for any given instance, 'Why?' explanations are minimal hitting sets of 'Why Not?' explanations and vice-versa. Furthermore, the paper devises novel algorithms for extracting and enumerating both forms of explanations.

==> algs/bls.tex <==
%------------------------------------------------------------------------------%
% File:        bls.tex
%------------------------------------------------------------------------------%
%
%
\SetKwFunction{tfunc}{{\sc ExtractCXp}} % 
%\Indm
\Func \tfunc{$\fml{M}_{\pi}$,$\fml{C}$, $\pi$} \;

\Indp
\KwIn{
  $\fml{F}_{\fml{M},\pi}$: ML model,
  $\fml{C}$: Input cube,
  $\pi$: Prediction
}
\KwOut{
  $\sigma$: Minimal set
}
\TopBlankLine
{
  \lnlset{a2:1}{1}
  $\sigma \gets \emptyset$ \tcp*[r]{$\sigma$ is under-approximation}
  \lnlset{a2:2}{2}
  \ForEach(\tcp*[f]{\textsl{Inv:}~$\sigma\entails\fml{M}_{\pi}$}){$u\in\fml{C}$}{
      \lnlset{a2:3}{3}
      \uIf(\tcp*[f]{$u$ ok?}){$\sigma\cup\{u\}\nentails\fml{M}_{\pi}$}{
        \lnlset{a2:4}{4}
        $\sigma \gets \sigma \cup \{u\}$ \tcp*[r]{If yes, expand $\sigma$} %\;
      }
    }
  \nlset{5}
  \Return $\fml{C}\setminus\sigma$ \tcp*[r]{$\fml{C}\setminus\sigma$ is CXp}
}
\Indm
\BotBlankLine
%
%------------------------------------------------------------------------------%

%
%------------------------------------------------------------------------------%


==> algs/del.tex <==
%------------------------------------------------------------------------------%
% File:        del.tex
%------------------------------------------------------------------------------%
%
\SetKwFunction{tfunc}{{\sc ExtractAXp}} %
%\Indm
\Func \tfunc{$\fml{M}_{\pi}$,$\fml{C}$, $\pi$} \;

\Indp
\KwIn{
  $\fml{M}_{\pi}$: ML model,
  $\fml{C}$: Input cube,
  $\pi$: Prediction
}
\KwOut{
  $\sigma$: Minimal set
}
\TopBlankLine
{
  \lnlset{a1:1}{1}
  $\sigma \gets \fml{C}$ \tcp*[r]{$\sigma$ is over-approximation}
  \lnlset{a1:2}{2}
  \ForEach(\tcp*[f]{\textsl{Inv:}~$\sigma\entails\fml{M}_{\pi}$}){$u\in\sigma$}{
      \lnlset{a1:3}{3}
      \uIf(\tcp*[f]{$u$~unneeded?}){$\sigma\setminus\{u\}\entails\fml{M}_{\pi}$}{
        \lnlset{a1:4}{4}
        $\sigma \gets \sigma \setminus \{u\}$ \tcp*[r]{If so, drop it} %\;
      }
    }
  \nlset{5}
  \Return $\sigma$ \tcp*[r]{$\sigma$ is AXp}
}
\Indm
\BotBlankLine
%
%------------------------------------------------------------------------------%


==> ddisc.tex <==
\paragraph{Discussion.}

Tim Miller writes,
\begin{quote}
Explanations are contrastive—they are sought in response to particular
counterfactual cases,which are termed {\em foils} in this paper.That
is,people do not ask why event P happened,but rather why event P
happened instead of some event Q.
\end{quote}



==> disc.tex <==
\section{Discussion} %\hfill??
\label{sec:disc}
\vspace*{-7pt}
Our results show that we are able to provide intuitively appealing
contrastive explanations automatically for the behavior of some ML
models.  However,  another important parameter for epistemic adequacy
of explanations is the characterization of the input data $X$ for a
learning algorithm. If the dimensionality of $X$ is too high or if the
dimensions don’t correspond to intuitive concepts, then our
constrastive explanations may not be satisfactory for humans.  To get
fully adequate contrastive explanations, it will be important in such
cases to find the right representation of the data.  Data
representation remains a problem for many approaches to explanations
of ML program behavior.

We also note that contrastive explanations may also express
adversarial examples that shift a prediction but for intuitively the
wrong reasons~\cite{kwiatkowska-tcs20}.  These might not be  good
explanations  of  the phenomenon the ML program is trying to model.
Nevertheless such contrastive explanations provide a valuable insight
into the workings of the program and its weaknesses  and can be as such very
valuable.


==> impact.tex <==
%\section*{Broad Impact}
\section*{Broader Impact}

Our paper deals with explanations of the predictions made by Machine
Learning (ML) models, and builds on a recent line of work on computing
logically sound explanations, which precisely capture the behavior of
the ML model, and which are also independently verifiable. We see such
explainability as a key factor in rendering AI more acceptable and
more accountable to the general public’s demands and fears. In
addition, we have provided algorithms that automatically provide
logically sound explanations answering important questions, e.g. why a
certain decision was not made by an ML algorithm. For example, our
explanations help a person who applied for a loan to understand why an
ML algorithm used by a bank came to the conclusion that he or she did
not get a loan.


Past work on rigorous approaches for XAI focused on answering `Why?’
questions, e.g.\ `Why prediction $\pi$?'.
%
In contrast, our paper investigates alternative types of explanations,
e.g.\ studied in recent work~\cite{miller-aij19},
and develops ways for computing logically sound
%rigorous model-based
explanations for `Why Not?' questions, e.g.\ `Why prediction $\pi$ and
not prediction $\delta$?'.

More importantly, our paper shows that explanations for `Why?' and
`Why Not?' questions are related by a duality relationship that can be
traced to past work on model-based diagnosis. This relationship allows
tapping on a wide range of algorithms but also, and more importantly,
reveals ways for efficiently enumerating explanations for both `Why?'
and `Why Not?' questions.

%In principle this could with the proper user interface (UI) allow anyone to get explanations of the behavior of an ML model.


% Our paper deals with explanations of the predictions made by Machine
% Learning (ML) models, and builds on a recent line of work on computing
% logically sound explanations, which precisely capture the behavior of
% the ML model, and which are also independently verifiable.
% %

% Past work on rigorous approaches for XAI focused on answering ‘Why?’
% questions, e.g.\ 'Why prediction $\pi$?'.
% %
% In contrast, our paper investigates alternative types of explanations,
% e.g.\ studied in recent work~\cite{miller-aij19},
% and develops ways for computing logically sound
% %rigorous model-based
% explanations for ‘Why Not?’ questions, e.g.\ 'Why prediction $\pi$ and
% not prediction $\delta$?'.

% More importantly, our paper shows that explanations for 'Why?' and
% 'Why Not?' questions are related by a duality relationship that can be
% traced to past work on model-based diagnosis. This relationship allows
% tapping on a wide range of algorithms but also, and more importantly,
% reveals ways for efficiently enumerating explanations for both 'Why?'
% and 'Why Not?' questions.

% \bigskip
% Vs.
% \bigskip

% Our paper deals with explanations of Machine Learning program behavior \nnote{Is it ok to change "program" to "model'?}.  By furnishing a rigorous and verifiable means for producing both contrastive and abductive explanations,
% \nnote{Small suggestion: By furnishing a rigorous and verifiable means for producing insightful explanations, i.e. contrastive and abductive,}
% we provide logically sound explanations of program behavior, which is an important contribution to efforts to make AI decisions explainable.  We see such explainability as a key factor in rendering AI more acceptable and more accountable to the general public's demands and fears.  In addition, we have provided algorithms that automatically provide logically sound explanations.  In principle this could with the proper user interface (UI) allow anyone to get explanations of the behavior of an ML model. Concretely, such a UI could help a user understand why an ML algorithm used by a bank came to the conclusion that he or she did not get a loan.

% There is also a close connection between what we have called contrastive explanations and fairness.  \nnote{It seems to me that we dive into new details of a new material for this high-level statement. I would I just keep the first paragraph as it clearly positions our work.What do you think?} One important approach to fairness involves counterfactuals---a decision or prediction is fair with respect to some protected feature $F$ and individual $x$, if were one to shift the value on $F$ keeping all other factors as similar to their original values on $x$ as possible, one would not change the prediction.  Our contrastive explanations precisely yield such counterfactuals and so we see our work as offering an automatic means for exploring the fairness of ML models.


==> texfigs/encoding0.tex <==
~
\vspace*{0.3cm}
%
\begin{equation*}
  \begin{array}{l}
    \left[%
      (\msf{L}=\msf{lng})\lor%
      (\msf{L}=\msf{shrt})\land(\msf{T}=\msf{flUp})\land(\msf{A}=\msf{ukwn})
      \right]\limply(\pi=\msf{skips})
    \land \\[2pt]
    \left[%
      (\msf{L}=\msf{shrt})\land(\msf{T}=\msf{new})\lor%
      (\msf{L}=\msf{shrt})\land(\msf{T}=\msf{flUp})\land(\msf{A}=\msf{kwn})
      \right]\limply(\pi=\msf{reads}) \\
  \end{array}    
\end{equation*}


==> xpiip.tex <==

\section{Understanding the Definition of Contrastive Explanation}

\paragraph{Relating with the work of Miller~\cite{miller-aij19}.}

The contrastive explanations we are computing answer the question:
\emph{Why ($\pi$ and) not $\neg\pi$}? A more general contrastive
explanation would be \emph{Why ($\pi$ and) not $\delta$}, with
$\pi\not=\delta$? Note that, since the prediction $\pi$ is given, what
we are only interested in changing the prediction to either $\neg\pi$
or $\delta$. We refer to answering the first question as a
\emph{basic} contrastive explanation, whereas answering the second
question will be referred to as a \emph{targeted} contrastive
explanation.

The duality result between AXp's and CXp's proved in the paper applies
only to basic contrastive explanations.
%
Contrastive explanations of the second form will be tagged with the
target prediction $\tn{CXp}_{\delta}$.

\paragraph{Computational complexity of finding $\tn{CXp}_{\delta}$.}

At first, answering the second question may seem computationally
harder than the answering the first question, since we want to pick a
set of literals of the original instance while ensuring a different
prediction.

Nevertheless, we can devise approaches for computing contrastive
explanations of the form $\tn{CXp}_{\delta}$ (i.e.\ answering the
second question above). Essentially, we want a pick of feature-value
pairs such that the prediction is $\delta$. We start by letting all
features to take any value, and such that the resulting prediction is
$\delta$. We then iteratively attempt fix feature-value pairs to those
in the instance, while the prediction remains $\delta$. This way, the
set of literals that change value are a subset-minimal set of
feature-value pairs that is sufficient for predicting $\delta$.

Given the above, we can compute targeted contrastive explanations with
a linear number of queries to an oracle deciding the decision problem
for (the encoding of) the ML model.

\paragraph{Alternative way to compute $\textbf{CXp}_{\bm{\delta}}$.}
%
One can adapt the logic-based formulation of \autoref{def:cxp} when
dealing with the compution of one $\tn{CXp}_{\delta}$, or with their
enumeration.
%
Assume that instance $\tau$ is classified by $\fml{M}$ as $\pi$, i.e.\
$\tau\land\fml{M}_\pi\entails\bot$.

Consider a pair $(\fml{B},\fml{R})$, where $\fml{R}\triangleq\tau$ and
$\fml{B}\triangleq\neg\fml{M}_{\pi}$.
%
Now, any MCS of formula $(\fml{B},\fml{R})$ restores its consistency,
i.e.\ it breaks the entailment $\tau\entails\fml{M}_\pi$ and ``makes''
a misclassification feasible.

In order to control what kind of misclassifiction is allowed and so to
focus only on a specific class $\delta\in\mbb{K}$, $\delta\neq\pi$,
one can apply additional constraints forbidding all other classes
$\rho\in\mbb{K}\setminus\{\pi,\delta\}$.
%
Concretely, $\fml{B}$ can be replaced with
$\fml{B}^\delta=\fml{B}\land\bigwedge_{\rho\in\mbb{K}\setminus\{\pi,\delta\}}\neg{\rho}$.
%
Now, an MCS of the pair $(\fml{B}^\delta,\fml{R})$ is a
$\tn{CXp}_{\delta}$.

Furthermore, instead of a concrete target class $\delta$, we can
consider a subset $\delta\in\Delta\subseteq\mathbb{K}$ of target
classes and consider computing MCSes of formula
$(\fml{B}^\Delta,\fml{R})$, with
$\fml{B}^\Delta=\fml{B}\land\bigwedge_{\rho\in\mbb{K}\setminus(\Delta\cup\{\pi\})}\neg{\rho}$.
%
Each such MCS determines a $\tn{CXp}_{\Delta}$, i.e.\ a contrastive
explanation targeting any of the classes of $\Delta\subseteq\mbb{K}$.

Any MCS computation or enumeration algorithm can be applied to
$(\fml{B}^\delta,\fml{R})$ or $(\fml{B}^\Delta,\fml{R})$.
%
Also, one $\tn{CXp}_{\delta}$ or $\tn{CXp}_{\Delta}$ can be computed
with a logarithmic number of oracle calls.

\paragraph{Prime implicants vs.\ prime implicates.}

Given earlier work~\cite{darwiche-ijcai18} on PI-explanations and
CM-explanations, a natural question would be to relate contrastive
explanations with a concept similar to PI-explanations or
CM-explanations.
%
Prime implicates seem to represent a natural candidate (as opposed to
prime implicants), where a prime implicate is a minimal set
$\eta\subseteq\tau$ of feature-value pairs sufficient for
$\neg\fml{M}_{\pi}$, i.e.\ $\eta\entails\neg\fml{M}_{\pi}$.

But this does not reflect what is expected of a contrastive
explanation~\cite{miller-aij19}, i.e.\ we want to know which literals
to change, such that the predicion changes. No entailment requirements
are specified.


\paragraph{On nomenclature.}

This paper defines rigorous explanations as subset-minimal sets of
feature-value pairs which are sufficient for the prediction. Thus,
such explanations answer a \emph{Why?} question, and are referred to
as \emph{abductive explanations} due to the connections with abduction
in AI.
%
Other names have been used to denote rigorous explanations of ML
models. These include
PI-explanations~\cite{darwiche-ijcai18,darwiche-aaai19} and minimal
sufficient reasons~\cite{darwiche-ecai20,darwiche-pods20}.
%
An alternative definition is CM-explanations~\cite{darwiche-ijcai18},
but these refer to cardinality minimal numbers of true/false literals,
and so have a different focus.


\paragraph{Additional relationships to investigates further.}

Earlier work~\cite{inms-aaai19} also addressed duality relationships
of explanations, but consider global explanations and their
relationship with counterexamples. However, any global explanation is
local to the instances with which it is compatible with. Hence, we can
relate counterexamples (and so adversarial examples) with global
abductive explanations, which are local for some instances, and so
which can be related with (local) contrastive explanations.


\paragraph{Should we revisit CXp's?}

While trying to clarify the ideas, it seemed that a different
definition of CXp could be more acceptable in practice:

\begin{definition}[Contrastive Explanation] \label{def:cxp}
  Given an instance $\tau$, with a prediction $\pi$, and an ML model
  represented by a predicate $\fml{M}_{\pi}$,
  i.e.\ $\tau\entails\fml{M}_{\pi}$, a \emph{contrastive
    explanation} is a minimal subset of literals of $\tau$,
  $\rho\subseteq\tau$, each replaced by literals from each feature
  domain to produce $\rho'$,
  such that $(\tau\setminus\rho)\land\rho'\entails\fml{M}_{\neg\pi}$.
\end{definition}


